Thales: Formulating and Estimating Architectural Vulnerability Factors for DNN Accelerators

As Deep Neural Networks (DNNs) are increasingly deployed in safety critical and privacy sensitive applications such as autonomous driving and biometric authentication, it is critical to understand the fault-tolerance nature of DNNs. Prior work primarily focuses on metrics such as Failures In Time (FIT) rate and the Silent Data Corruption (SDC) rate, which quantify how often a device fails. Instead, this paper focuses on quantifying the DNN accuracy given that a transient error has occurred, which tells us how well a network behaves when a transient error occurs. We call this metric Resiliency Accuracy (RA). We show that existing RA formulation is fundamentally inaccurate, because it incorrectly assumes that software variables (model weights/activations) have equal faulty probability under hardware transient faults. We present an algorithm that captures the faulty probabilities of DNN variables under transient faults and, thus, provides correct RA estimations validated by hardware. To accelerate RA estimation, we reformulate RA calculation as a Monte Carlo integration problem, and solve it using importance sampling driven by DNN specific heuristics. Using our lightweight RA estimation method, we show that transient faults lead to far greater accuracy degradation than what todays DNN resiliency tools estimate. We show how our RA estimation tool can help design more resilient DNNs by integrating it with a Network Architecture Search framework.

==> back.tex <==
\section{Background}
\label{sect:back}

%We first describe the scope of error resilience that this focuses on, i.e., radiation-induced soft errors~\cite{??} (\Sect{sect:back:transient}). We then discuss a particular metric that this paper uses to quantify the impact of transient errors on DNN accuracy (\Sect{sect:back:ra}). 

\paragraph{Scope of Work: Transient Errors}
This paper specifically focuses on transient errors, which are radiation-induced accidental bit flips~\cite{seifert2006radiation,seifert2010radiation,srinivasan1994accurate}. While such bit flips can happen anywhere on a chip~\cite{naseer2007critical,jahinuzzaman2009soft,degalahal2003analyzing,lantz1996soft, rech2012neutron,de2015evaluation}, we focus on FFs, since other memory structures such as SRAM and DRAM are usually protected by error detection and correction bits~\cite{slayman2005cache,chen1984error}. Transient errors in FFs are also commonly used to emulate transient errors in combinational logic~\cite{??}.

%Transient errors threat the reliability of DL accelerators which is critical as many DL accelerators now have been utilized in applications such as autonomous vehicles~\cite{hu2019dynamic}. Transient errors can potentially influence flip flops in the data loading path of DL accelerators, the processing elements of DL accelerators and the write back path. Such influences can be translated to algorithm-level wrong inputs, weights, bias, partial sums and outputs. Finally, the wrong outputs will cause a degradation on the accuracy of the applications which may lead to safety concerns.    

\paragraph{Quantifying the Impact of Transient Error}
In the circuit literature, the most common metric for quantifying the impact of transient errors is the Failures In Time (FIT) rate of a device (accelerator). The FIT rate, intuitively, quantifies \textit{how often} a device fails, which in the case of a DNN accelerator could be either the DNN mis-predicts or system anomaly such as a crash~\cite{he2020fidelity}.

This paper focuses on a complementary metric, which, intuitively, quantifies the accuracy of a DNN \textit{given} that a transient error occurs. We call this metric Resiliency Accuracy (RA).
In other words, RA gives a measure as to how accurate an inference is when the underlying accelerator is affected by a transient error. A higher RA indicates that a DNN is more resilient to soft errors, and vice versa. Accurately estimating RA is important: it enables developing algorithms and architectures that are more resilient to soft errors from ground up.

Without losing generality, a DNN's RA can be defined as:

\begin{align}
    RA = \sum_{i=1}^{N}p_{i}RA_{i}
\end{align}

\noindent where $N$ is the total number of \textit{fault sites};


==> future.tex <==
\section{Discussions}
\label{sec:future}

\paragraph{Limitations.} Our RA estimation framework assumes that a DNN's data reuse is regular: all variables of the same type in a layer have the same reuse.
%This assumption allows us to derive the software fault site probability using the simple analytical model in \Equ{eq:pequ}.
This assumption does not hold for Graph Neural Networks~\cite{scarselli2008graph,shchur2018pitfalls,zhang2019heterogeneous} and point cloud DNNs~\cite{zhang2021point,tiator2020point,zhou2018voxelnet,qi2017pointnet}, where data reuses are not uniform because of the irregular connections in graphs and/or neighbor searches~\cite{tao2002continuous,jegou2010product,seidl1998optimal, xu2019tigris, feng2022crescent, zhu2022rtnn}.

%Absent RTL-level utilization data, we assume that the MAC array in a DNN accelerator is nearly fully utilized, which might not hold when the accelerator has a large MAC array but the compute requirement is low (e.g., a small layer) or when using an unbalanced hardware design that is bottlenecked by memory accesses. The $UF(T_j)$ term in \mbox{\Equ{eq:raequ}} could be populated with the actual utilization data, when available, to improve the RA estimation accuracy as shown in \mbox{\Sect{sec:val:prob}}.

%\paragraph{Importance Sampling Heuristics.} While our importance sampling methods are effective, their efficiency could be further improved by incorporating network-specific knowledge. For instance, one could consider the impact of different layers in a DNN. On one hand, bit flips in earlier layers could degrade the inference accuracy more than those in later layers, because a bit flip in an earlier layer gets propagated to more weights/activations in a model. On the other hand, faults in later layers are less likely to be masked (e.g., by ReLU) than those in earlier layers. It would be interesting to profile the layer-wise impact of transient faults on RA, and use the profiling results to derive better sampling PDFs.

%\mode{IS-BL}: this is importance sampling using the BP+Layer heuristic discussed in \Sect{sec:sampling:is}. Based on our profiling results, we add 10\% accuracy drop in $A(j)$ for software faults sites that are in the first 2 layers in AlexNet and first 10 layers in MobileNet and YOLOv3.

\paragraph{Input Diversity.} As with SA, a network's RA is necessarily obtained with respect to a given training set and a given test set.
Recent work by Mahmoud et al.~\cite{mahmoud2021optimizing} shows that the vulnerability of an inference varies with the input image. Therefore, it is expected that a network's RA would change under a different test set or if the input distribution in deployment is different from that of the training set --- the same issue that normal DNN training faces.
%The goal of our paper is to estimate the RA of a \textit{given} network on a \textit{given} test set.
%If a network is trained on a more representative training set, \proj can be readily used to provide a more representative RA estimation.

%\hl{In this sense, Thales provides a new perspective to improving the representativeness of a training set: the training set should ideally have a RA similar to that of the test set. Today, the representativeness of a training set is discussed in the context of SA. Taking the CIFAR-10 dataset as an example, we show that the RA drops from the training set to the test set by 1.4\% for MobileNet and by 2.1\% for AlexNet, motivating future work to improve the resiliency-oriented representativeness of a training set.}

%For this I obtained data for MobileNet and AlexNet (as I though they are more realistic networks). So for them, SA drop (training set vs test set)  is 6.4% and 17.3 % respectively. Whereas the RA drop (training set vs test set) is 1.37 % and 2.12 % respectively.






















==> rev.tex <==
\section{Revision Letter}

\subsection{Major revisions asked in the meta review}

\vspace{5pt}
\noindent \textbf{Better explanation of the definitions, assumptions, and calculations of the RA metric which seems to be unclear and in doubt. (A, B, C, E, F)}

See revision in \Sect{sec:motivation:metric}.

\vspace{10pt}
\noindent \textbf{Characterization of the impact of faults in the control FFs and the likelihood of crashes vs. inaccurate inference results. (E)}

See revision in \Sect{sec:robust:fs} for an explanation of what control FFs are and how they affect DNN accuracy.

See revision in \Sect{sec:ra:anal} for the RA results that separate the effect of control FFs.

\vspace{10pt}
\noindent \textbf{Comparison and discussion vs. prior publications (mainly \cite{he2020fidelity} and \cite{li2017understanding}) and clear explanation of the novelty this paper brings. (B, C)}

See revision in \Sect{sec:ra:sample} for a quantitative comparison with \cite{mahmoud2021optimizing}.

We rewrite the Related Work (\Sect{sec:related}) to discuss the fundamental novelty of our work over \cite{he2020fidelity}, \cite{li2017understanding}, and \cite{mahmoud2021optimizing}.

\vspace{10pt}
\noindent \textbf{Support of claims for inaccuracies of previous works. (B)}

We previously, in Introduction and \Sect{sec:motivation:sw}, say that today’s model-level tools assume that all the software fault sites have equal faulty probability. We acknowledge that ``today’s model-level tools'' is too broad and vague. We meant to refer to three specific tools: TensorFI~\cite{chen2020tensorfi}, PytorchFI~\cite{mahmoud2020pytorchfi}, and Ares~\cite{reagen2018ares}. \cite{mahmoud2021optimizing}, which is built on top of PytorchFI, does not make such assumptions. Accordingly, we made the following revisions.

First, we remove the vague language ``today’s model-level tools'' in both the Introduction and \Sect{sec:motivation:sw}. The text now explicitly names the three tools that make that assumption.

Second, we also quote texts, verbatim, from TensorFI~\cite{chen2020tensorfi}, PytorchFI~\cite{mahmoud2020pytorchfi} to show that they indeed make that assumption. See the footnote in \Sect{sec:motivation:sw} (page 3).

Finally, we also acknowledge, in \Sect{sec:ra:sample}, that \cite{mahmoud2021optimizing}, instead of performing uniform sampling, weighs different activations based on the MACs used to compute the activation out. We provide a quantitative comparison with such a sampling strategy in \Sect{sec:ra:sample}.

\vspace{10pt}
\noindent \textbf{Explanation of what is the ground truth in the evaluation part (``exhaustive RTL simulation'' is unclear). (A, C, D)}

See revision in \Sect{sec:val} for a description of exhaustive RTL simulation.

See revision in \Sect{sec:ra:setup} for how we obtain the ground truth for evaluation.

\subsection{Other revisions}

\vspace{5pt}
\noindent \textbf{How do you know the importance of different bits in the BP-aware heuristic? (A)}

See revision in \Sect{sec:ra:sample}. Note that the bit-level importance is a heuristics that affects convergence not correctness.

\vspace{10pt}
\noindent \textbf{How can one use the RA estimate if the input distribution is different from the train set distribution? (B)}

See revision at the end of \Sect{sec:future}.

\vspace{10pt}
\noindent \textbf{Does Thales consider only single-bit faults in FFs (no multi-bit faults and no SRAMs)? How about MAC logic faults? (B, C, E)}

See revision in \Sect{sec:motivation:metric}, under \textbf{Assumptions}.

\vspace{10pt}
\noindent \textbf{Faults are not uniform across fault sites (B, E, F)}

Agreed. We revise the RA equation (\Equ{eq:RA}) to reflect non-uniform raw FIT rates. We also clarify in \Sect{sec:motivation:metric}, under \textbf{Assumptions}, that we assume all bit positions have same faulty probability as with prior work such as~\cite{mahmoud2021optimizing}.

\vspace{10pt}
\noindent \textbf{Comment on the similarities of your findings to Papadimitriou and Gizopoulos~\cite{papadimitriou2021demystifying} and comments on a common formalization for both CPU and NPU (and possibly GPU). (D)}

See revision at the end of \Sect{sec:related}.


























